Adversarial Sub-sequence for Text Generation

Generative adversarial nets (GAN) has been successfully introduced for generating text to alleviate the exposure bias. However, discriminators in these models only evaluate the entire sequence, which causes feedback sparsity and mode collapse. To tackle these problems, we propose a novel mechanism. It first segments the entire sequence into several sub-sequences. Then these sub-sequences, together with the entire sequence, are evaluated individually by the discriminator. At last these feedback signals are all used to guide the learning of GAN. This mechanism learns the generation of both the entire sequence and the sub-sequences simultaneously. Learning to generate sub-sequences is easy and is helpful in generating an entire sequence. It is easy to improve the existing GAN-based models with this mechanism. We rebuild three previous well-designed models with our mechanism, and the experimental results on benchmark data show these models are improved significantly, the best one outperforms the state-of-the-art model.\footnote[1]{All code and data are available at https://github.com/liyzcj/seggan.git

==> reference.tex <==
\section*{References}

[1] S. Bengio, O. Vinyals, N. Jaitly, and N., Shazeer. Scheduled sampling for sequence prediction with recurrent neural networks. In \textit{NIPS}, 1995.

[2] T. Che, Y. Li, R. Zhang, R. D. Hjelm, W. Li, Y. Song, and Y. Bengio. Maximum-likelihood augmented discrete generative adversarial networks. \textit{arXiv preprint arXiv:1702.07983}, 2017.

[3] T. Che, Y. Li, A. P. Jacob, Y. Bengio, and W. Li. Mode regularized generative adversarial networks. In \textit{ICLR}, 2017.

[4] L. Chen, S. Dai, C. Tao, D. Shen, Z. Gan, H. Zhang, Y. Zhang and L. Carin. Adversarial text generation via feature-mover’s distance. In \textit{NIPS}, 2017.

[5] W. Fedus, I. Goodfellow, and A. Dai. Maskgan: Better text generation via filling in the \underline{\quad}. In \textit{ICLR}, 2018.

[6] I. Goodfellow, J. Pouget-Abadie, M. Mirza, B. Xu, D. Warde-Farley, S. Ozair, A. Courville, and Y. Bengio. Generative adversarial nets. In \textit{NIPS}, 2014.

[7] J. Guo, S. Lu, H. Cai, W. Zhang, Y. Yu, and J. Wang. Long text generation via adversarial training with leaked information. In \textit{AAAI}, 2018.

[8] S. Hochreiter, and J. Schmidhuber. (1997) Long short-term memory. {\it Neurocomputing} {\bf 9}(8):1735-1780.

[9] E. Jang, S. Guo, and B. Poole. Categorical reparameterization with gumbel-softmax. \textit{arXiv preprint arXiv:1611.01144}, 2016.

[10] J. Li, W. Monroe, T. Shi, A. Ritter and D. Jurafsky. Adversarial learning for neural dialogue generation. In \textit{EMNLP}, 2017.

[11] K. Lin, D. Li, X. He, Z. Zhang, and M.-T, Sun. Adversarial ranking for language generation. In \textit{NIPS}, 2017.

[12] Y. Liu, Z. Qin, Z. and H. Luo. (2018) Auto-painter: Cartoon image generation from sketch by using conditional Wasserstein generative adversarial networks. {\it Neurocomputing} {\bf 311}(x):78-87.

[13] C. J. Maddison, A. Mnih, and Y. W. Teh. The concrete distribution: A continuous relaxation of discrete random variables. In \textit{ICLR}, 2017.

[14] W. Nie, N. Narodytska, and A. Patel. RelGAN: Relational Generative Adversarial Networks for Text Generation. In \textit{ICLR}, 2019.

[15] K. Papineni, S. Roukos, T. Ward, and W.-J. Zhu. Bleu: a method for automatic evaluation of machine translation. In \textit{ACL}, 2002.

[16] S. Semeniuta, A. Severyn, and S. Gelly. On accurate evaluation of gans for language generation. arXiv preprint arXiv:1806.04936, 2018.

[17] Z. Shi, X. Chen, X. Qiu and X. Huang. Toward Diverse Text Generation with Inverse Reinforcement Learning. In \textit{IJCAI}, 2018.

[18] D. Silver, A. Huang, C. J. Maddison, A. Guez, L. Sifre, et al. 2016. Mastering the game of go with deep neural networks and tree search. Nature 529(7587):484–489

[19] A. Srivastava, L. Valkov, C. Russell, M. U. Gutmann and C. Sutton. VEEGAN: Reducing Mode Collapse in GANs using Implicit Variational Learning. In \textit{NIPS}, 2016.

[20] S. Subramanian, S. Rajeswar, F. Dutil, C. Pal, and A. Courville. Adversarial Generation of Natural Language. In \textit{the 2nd Workshop on Representation Learning for NLP}, 2017.

[21] L. Theis, A.Oord, and M. Bethge. A note on the evaluation of generative models. In \textit{ICLR}, 2016.

[22] A. Vaswani, N. Shazeer, N. Parmar, J. Uszkoreit, L. Jones, A. N. Gomez, Ł. Kaiser, and I. Polosukhin. Attention is all you need. In \textit{NIPS}, 2017.

[23] Y. Wu, M. Schuster, Z. Chen, Q. V. Le, M. Norouzi, W. Macherey, M. Krikun, Y. Cao, Q. Gao, K. Macherey, J. Klingner, A. Shah, M. Johnson, X. Liu, L. Kaiser, S. Gouws, Y. Kato, T. Kudo, H. Kazawa, K. Stevens, G. Kurian, N. Patil, W. Wang, C. Young, J. Smith, J. Riesa, A. Rudnick, O. Vinyals, G. Corrado, M. Hughes, and J. Dean. Google’s neural machine translation system: Bridging the gap between human and machine translation. CoRR, abs/1609.08144, 2016.

[24] J. Xu, X. Ren, J. Lin and X. Sun. Diversity-Promoting GAN: A Cross-Entropy Based Generative Adversarial Network for Diversified Text Generation. In \textit{EMNLP}, 2018. 

[25] L. Yu, W. Zhang, J. Wang, and Y. Yu. SeqGAN: Sequence generative adversarial nets with policy gradient. In \textit{AAAI}, 2017.

[26] Y. Zhang, Z. Gan, K. Fan, Z. Chen, R. Henao, D. Shen, and L. Carin. Adversarial feature matching for text generation. In \textit{ICML}, 2017.

[27] Y. Zhu, S. Lu, L. Zheng, J. Guo, W. Zhang, J. Wang, and Y. Yu. Texygen: A Benchmarking Platform for Text Generation Models. In \textit{SIGIR}, 2018.
